Large-Scale Gravitational Lens Modeling with Bayesian Neural Networks for Accurate and Precise Inference of the Hubble Constant

We investigate the use of approximate Bayesian neural networks (BNNs) in modeling hundreds of time-delay gravitational lenses for Hubble constant ($H_0$) determination. Our BNN was trained on synthetic HST-quality images of strongly lensed active galactic nuclei (AGN) with lens galaxy light included. The BNN can accurately characterize the posterior PDFs of model parameters governing the elliptical power-law mass profile in an external shear field. We then propagate the BNN-inferred posterior PDFs into ensemble $H_0$ inference, using simulated time delay measurements from a plausible dedicated monitoring campaign. Assuming well-measured time delays and a reasonable set of priors on the environment of the lens, we achieve a median precision of $9.3$\% per lens in the inferred $H_0$. A simple combination of 200 test-set lenses results in a precision of 0.5 $\textrm{km s}^{-1} \textrm{ Mpc}^{-1}$ ($0.7\%$), with no detectable bias in this $H_0$ recovery test. The computation time for the entire pipeline -- including the training set generation, BNN training, and $H_0$ inference -- translates to 9 minutes per lens on average for 200 lenses and converges to 6 minutes per lens as the sample size is increased. Being fully automated and efficient, our pipeline is a promising tool for exploring ensemble-level systematics in lens modeling for $H_0$ inference.

==> Makefile <==
# To make the document with the default settings:
# > make
#
# To make with a specific format:
# > make <format>
#
# To tar up a flat version of a specific format:
# > make <format> tar
#
# Alex Drlica-Wagner: https://github.com/LSSTDESC/start_paper/issues/new?body=@kadrlica

# Primary file names - avoid cookiecutter variables, to enable `make
# upgrade` to cleanly over-write this Makefile...
main ?= main
#default=$(shell cat .metadata.json | grep 'default_format' | cut -d'"' -f4)
outname ?= $(notdir $(shell pwd))

#ifeq ($(default), {{ cookiecutter.default_format }})
style ?= lsstdescnote
#else
# style=${default}
#endif

# 'note' shall be an alias for 'lsstdescnote'
ifeq ($(style),note)
style = lsstdescnote
endif
# mkauthlist doesn't recognize lsstdescnote as a style, so tell it to do something generic
ifeq ($(style),lsstdescnote)
mastyle = tex
else
mastyle = $(style)
endif

DESCTEX := desc-tex
DESCTEXORIGIN := https://github.com/LSSTDESC/desc-tex.git
LSSTTEX := lsst-texmf
LSSTTEXORIGIN := https://github.com/lsst/lsst-texmf.git

localpip ?= F
PIPOPTS = --upgrade-strategy only-if-needed
ifeq ($(localpip),T)
MKAUTHBIN := bin/mkauthlist
MKAUTH := PYTHONPATH=$$(ls -d lib/python*/site-packages 2>/dev/null | head -n1):$$PYTHONPATH $(MKAUTHBIN)
PIPOPTS += --install-option="--prefix=$(PWD)"
GETMKAUTH := [ -e $(MKAUTHBIN) ] || pip install $(PIPOPTS) mkauthlist
else
MKAUTHBIN :=
MKAUTH := mkauthlist 
GETMKAUTH := pip list 2>/dev/null | grep -q mkauthlist || pip install $(PIPOPTS) mkauthlist
endif

# LATEX environment variables
export TEXINPUTS:=./$(DESCTEX)/styles/:./tables/:
export BSTINPUTS:=./$(DESCTEX)/bst/:
export BIBINPUTS:=./$(DESCTEX)/bib/:./$(LSSTTEX)/texmf/bibtex/bib/:

# LaTeX journal class switcher flags
# apj=\def\flag{apj}
# apjl=\def
# mnras=\def\flag{mnras}

# Submission flags (these need some thought)
# arxiv=\def\flag{emulateapj}
# submit=${aastex}
# draft=\def\linenums{\linenumbers}

# Files to copy when making tarball
tardir := tmp
figdir ?= ./figures
figures ?= $(figdir)/*.{png,jpg,pdf}
tabdir ?= ./tables
tables ?= $(tabdir)/*.tex
styles ?= ./$(DESCTEX)/styles/*.{sty,cls}
bibs ?= ./$(DESCTEX)/bib/*.bst
source = $(main).{tex,bbl,bib} $(DESCTEX)/bib/lsstdesc.bib $(DESCTEX)/ack/*.tex authors.tex contributions.tex $(LSSTTEX)/texmf/bibtex/bib/lsst.bib $(LSSTTEX)/texmf/bibtex/bib/lsst-dm.bib

tarfiles = $(figures) $(tables) $(styles) $(bibs) $(source)

# prefix for difference files
DIFPRE ?= diff_
# git repo branch to compare changes against
BASEBRANCH ?= master
# git repo branch we are compiling
THISBRANCH := $(shell git branch --no-color 2> /dev/null | sed -e '/^[^*]/d' -e 's/* \(.*\)/ \1/' | tr -d ' ')
# temp file for the version to compare against
DRAFT = $(main).$(BASEBRANCH)
# base for difference files to generate
DIFF = $(DIFPRE)$(THISBRANCH)--$(BASEBRANCH)


maketargets := all authlist clean copy diff help $(main) update tar templates tidy touch
.PHONY: $(maketargets)

styleopts := aastex61 apj apjl emulateapj lsstdescnote mnras note prd prl tex 
help:
	@echo "Usage: make [style=lsstdescnote] [localpip=F] <target(s)>\n Possible targets: $(maketargets) <style> $(DESCTEX) $(LSSTTEX)\n  all: equivalent to 'make $(main) copy'\n  authlist: use mkauthlist to generate latex author/affiliation listing\n  clean: remove latex temporary files AND compiled outputs\n  copy: copy $(main).pdf to $(outname).pdf\n  diff: if we're in a git repo, use latexdiff to compare the current $(main).tex vs the $(BASEBRANCH) branch, and attempt to compile to $(DIFF).pdf\n  help: what you're looking at\n  $(main): compile $(main).tex\n  update: update desc-tex, mkauthlist, and templates repo\n  tar: tar up latex source files to $(outname).tar.gz\n  templates: download latest templates to templates/\n  tidy: delete latex temporary files\n  touch: touch $(main).tex to force a recompile\n  <style>: equivalent to 'make style=<style> $(main) copy tar' (see style option)\n  $(DESCTEX): download $(DESCTEX), which provides the DESC header logo and latex helper files (done automatically on first latex compilation)\n  $(LSSTTEX): download $(LSSTTEX), providing (among other things) LSST project bib files (not done automatically)\n Options for style: $(styleopts) (Anything else results in generic latex)\n Options for localpip: T or F. Set to T to install mkauthlist in this directory rather than systemwide"


# Interpret `make` with no target as `make tex` (a latex Note).
# At present, if the default_format is anything other than
# [apj|apjl|mnras|prd|prl|emulateapj], a latex Note is made.
# In future, we could think of using `make` to eg run the ipynb
# notebook and make PDF from the output, but this has not been
# implemented yet.
$(main): export flag = \def\flag{${style}}
envflag = \\def\\flag{${style}}
all: $(main) copy

copy:
	cp ${main}.pdf ${outname}.pdf

touch:
	touch ${main}.tex

# if we are in a git repo, add as a submodule; otherwise clone
$(DESCTEX):
	if [ -d .git ]; then git submodule add $(DESCTEXORIGIN); else git clone $(DESCTEXORIGIN); fi
$(LSSTTEX):
	if [ -d .git ]; then git submodule add $(LSSTTEXORIGIN); else git clone $(LSSTTEXORIGIN); fi

#http://journals.aas.org/authors/aastex/linux.html
#change the compiler call to allow a "." file
# {% raw %}
$(main) : $(DESCTEX) authlist
	STYLEFLAG=$(envflag) latexmk $(main)
#	latexmk -g -pdf  \
	-pdflatex='openout_any=a pdflatex %O -interaction=nonstopmode "${flag}\input{%S}"'  \
	${main}
# {% endraw %}

diff: $(DIFF).pdf
$(DIFF).pdf: $(DIFF).tex
	STYLEFLAG=$(envflag) latexmk $<
$(DIFF).tex: $(DRAFT).tex $(main).tex
	latexdiff --exclude-textcmd="multicolumn" $^ > $@
# this ensures that the version to latexdiff against is always updated
.PHONY: $(DRAFT).tex
$(DRAFT).tex:
	if git show $(BASEBRANCH):$(main).tex > $@; then true; else echo "\n\n'make diff' is intended to be used inside a git repository\n"; false; fi



tar : $(main)
	mkdir -p ${tardir}
	cp ${tarfiles} ${tardir} | true
	cp ${outname}.pdf ${tardir}/${outname}.pdf
	cd ${tardir} && tar -czf ../${outname}.tar.gz . && cd ..
	rm -rf ${tardir}

authlist: authors.tex
authors.tex : authors.csv
	$(GETMKAUTH)
	$(MKAUTH) -j ${mastyle} -f -c "LSST Dark Energy Science Collaboration" \
		--cntrb contributions.tex authors.csv authors.tex
#	pip install --upgrade mkauthlist


# http://stackoverflow.com/q/8028314/
.PHONY: $(styleopts)
$(styleopts): export style = $(@)
$(styleopts): export flag = \def\flag{$(@)}
$(styleopts):
	$(MAKE) -e $(main)
	$(MAKE) -e copy
	$(MAKE) -e tar
# NB. the 'tex' target doesn't actually do anything in docswitch - make
# with no target compiles PDF out of main.tex using lsstdescnote.cls
# (which is to say, by default we assume you are writing an LSST
# DESC Note in latex format).

tidy:
	rm -f *.log *.aux *.out *.dvi *.synctex.gz *.fdb_latexmk *.fls
	rm -f *.bbl *.blg *Notes.bib ${main}.pdf

clean: tidy
	rm -f ${outname}.pdf ${outname}.tar.gz

# Update the tex styles etc:

baseurl=https://raw.githubusercontent.com/LSSTDESC/start_paper/deploy

# UPDATES=\
# texmf/bib/apj.bst \
# texmf/bib/mnras.bst \
# texmf/styles/aas_macros.sty \
# texmf/styles/aastex.cls \
# texmf/styles/aastex61.cls \
# texmf/styles/aps_macros.sty \
# texmf/styles/docswitch.sty \
# texmf/styles/emulateapj.cls \
# texmf/styles/mnras.cls \
# texmf/styles/lsstdescnote.cls \
# texmf/styles/lsstdesc_macros.sty \
# texmf/logos/desc-logo-small.png \
# texmf/logos/desc-logo.png \
# texmf/logos/header.png \
# lsstdesc.bib \
# .travis.yml \
# figures/example.png

# .PHONY: $(UPDATES)
# $(UPDATES):
# 	curl -s -S -o $(@) ${baseurl}/$(@)
# 	@echo " "

update: templates
	@echo Updating desc-tex
	cd $(DESCTEX) && git pull
	@echo
	@echo Updating mkauthlist
	pip install --upgrade $(PIPOPTS) mkauthlist
#@echo "\nOver-writing LaTeX style files with the latest versions: \n"
#@mkdir -p .logos figures texmf/styles texmf/bib
#$(MAKE) $(UPDATES)

# Get fresh copies of the templates etc, for reference:
# It is a bad idea to make these phony targets

TEMPLATES:=\
authors.csv \
main.ipynb \
main.md \
main.rst \
main.tex \
main.bib \
Makefile
#.metadata.json \
#.travis.yml 
#figures/example.png
# #acknowledgments.tex \

ALLTEMPLATES := $(TEMPLATES) header.png

# .PHONY: $(TEMPLATES)
# $(TEMPLATES):
# 	curl -s -S -o templates/$(@) ${baseurl}/$(@)
# 	@echo " "

gettemplates := $(foreach t,$(TEMPLATES),curl -s -S -o templates/$(t) ${baseurl}/$(t); )

# NB: fetching header.png will fail as long as desc-tex is private
templates:
	@echo "\nDownloading the latest versions of the template files, for reference: \n"
	@mkdir -p templates
	$(gettemplates)
	curl -f -s -S -o templates/header.png https://raw.githubusercontent.com/LSSTDESC/desc-tex/master/logos/header.png || true
	@echo
	@echo templates/ listing:
	@ls -a templates/*
	@for f in $(ALLTEMPLATES); do diff -q $$f templates/$$f; true; done
#$(MAKE) $(TEMPLATES)
#	$(MAKE) new

# Get a template copy of the latest Makefile, for reference:
# new:
# 	@echo "\nDownloading the latest version of the Makefile, for reference: \n"
# 	@mkdir -p templates
# 	curl -s -S -o templates/Makefile ${baseurl}/Makefile
# 	@echo " "

# Over-write this Makefile with the latest version:
# Why would we include this when a safe option already exists?
# upgrade:
# 	@echo "\nDownloading the latest version of the Makefile: \n"
# 	curl -s -S -o Makefile ${baseurl}/Makefile
# 	@echo "\nUpgrading version of mkauthlist: \n"
# 	pip install mkauthlist --upgrade --no-deps
# 	@echo "\nNow get the latest styles and templates with\n\n    make update\n    make templates\n"


==> authors.tex <==



==> contributions.tex <==



==> desc-tex/ack/key.tex <==
The DESC acknowledges ongoing support from the Institut National de Physique Nucl\'eaire et de Physique des Particules in France; the Science \& Technology Facilities Council in the United Kingdom; and the Department of Energy, the National Science Foundation, and the LSST Corporation in the United States.  DESC uses resources of the IN2P3 Computing Center (CC-IN2P3--Lyon/Villeurbanne - France) funded by the Centre National de la Recherche Scientifique; the National Energy Research Scientific Computing Center, a DOE Office of Science User Facility supported by the Office of Science of the U.S.\ Department of Energy under Contract No.\ DE-AC02-05CH11231; STFC DiRAC HPC Facilities, funded by UK BIS National E-infrastructure capital grants; and the UK particle physics grid, supported by the GridPP Collaboration.  This work was performed in part under DOE Contract DE-AC02-76SF00515.


==> desc-tex/ack/standard.tex <==
The DESC acknowledges ongoing support from the Institut National de Physique Nucl\'eaire et de Physique des Particules in France; the Science \& Technology Facilities Council in the United Kingdom; and the Department of Energy, the National Science Foundation, and the LSST Corporation in the United States.  DESC uses resources of the IN2P3 Computing Center (CC-IN2P3--Lyon/Villeurbanne - France) funded by the Centre National de la Recherche Scientifique; the National Energy Research Scientific Computing Center, a DOE Office of Science User Facility supported by the Office of Science of the U.S.\ Department of Energy under Contract No.\ DE-AC02-05CH11231; STFC DiRAC HPC Facilities, funded by UK BIS National E-infrastructure capital grants; and the UK particle physics grid, supported by the GridPP Collaboration.  This work was performed in part under DOE Contract DE-AC02-76SF00515.


==> desc-tex/ack/standard_short.tex <==
DESC acknowledges ongoing support from the IN2P3 (France), the STFC (United Kingdom), and the DOE, NSF, and LSST Corporation (United States).  DESC uses resources of the IN2P3 Computing Center (CC-IN2P3--Lyon/Villeurbanne - France) funded by the Centre National de la Recherche Scientifique; the National Energy Research Scientific Computing Center, a DOE Office of Science User Facility supported under Contract No.\ DE-AC02-05CH11231; STFC DiRAC HPC Facilities, funded by UK BIS National E-infrastructure capital grants; and the UK particle physics grid, supported by the GridPP Collaboration.  This work was performed in part under DOE Contract DE-AC02-76SF00515.


==> latexmkrc <==
# Choose which style to pass to docswitch
# NB: Default value here is always used by Overleaf
$theflag = $ENV{'STYLEFLAG'} || '\def\flag{lsstdescnote}';

# Set environment variables to search for tex inputs
# http://tex.stackexchange.com/a/50847/121099
$ENV{'TEXINPUTS'}='./desc-tex/:./tables/:' . $ENV{'TEXINPUTS'};
$ENV{'BSTINPUTS'}='./desc-tex/bib/:' . $ENV{'BSTINPUTS'};

# Set control tools
$go_mode = 1;
$pdf_mode = 1;
# You can change the \flag value here...
$pdflatex = 'openout_any=a pdflatex %O -interaction=nonstopmode "' . $theflag . '\input{%S}"'

